IMDPrompter: Adapting SAM to Image Manipulation Detection by Cross-View Automated Prompt Learning

Using extensive training data from SA-1B, the Segment Anything Model (SAM) has demonstrated exceptional generalization and zero-shot capabilities, attracting widespread attention in areas such as medical image segmentation and remote sensing image segmentation. However, its performance in the field of image manipulation detection remains largely unexplored and unconfirmed. There are two main challenges in applying SAM to image manipulation detection: a) reliance on manual prompts, and b) the difficulty of single-view information in supporting cross-dataset generalization. To address these challenges, we develops a cross-view prompt learning paradigm called IMDPrompter based on SAM. Benefiting from the design of automated prompts, IMDPrompter no longer relies on manual guidance, enabling automated detection and localization. Additionally, we propose components such as Cross-view Feature Perception, Optimal Prompt Selection, and Cross-View Prompt Consistency, which facilitate cross-view perceptual learning and guide SAM to generate accurate masks. Extensive experimental results from five datasets (CASIA, Columbia, Coverage, IMD2020, and NIST16) validate the effectiveness of our proposed method.

==> sec/0_abstract.tex <==
\begin{abstract}
% Using a vast amount of training data from SA-1B, the Segment Anything Model (SAM) has demonstrated outstanding generalization and zero-shot capabilities. However, as an instance segmentation method independent of categories, SAM heavily relies on manual priors, including points, boxes, and coarse-grained masks. Furthermore, its performance on tasks related to image manipulation detection has largely remained unexplored and unconfirmed. This paper aims to develop an image manipulation detection method based on the basic SAM model and incorporating various semantic-agnostic noisy graph information. Drawing inspiration from prompt learning, we propose a method called IMDPrompter, which learns to generate appropriate prompts for SAM, enabling it to generate accurate manipulation region masks for image manipulation detection. Extensive experimental results from five datasets, namely CASIA, Columbia, Coverage, IMD2020, and NIST16, validate the effectiveness of the proposed method.

Using extensive training data from SA-1B, the Segment Anything Model (SAM) has demonstrated exceptional generalization and zero-shot capabilities, attracting widespread attention in areas such as medical image segmentation and remote sensing image segmentation. However, its performance in the image manipulation detection field remains largely unexplored and unconfirmed. There are two main challenges in applying SAM to image manipulation detection: a) SAM heavily relies on prior manual guidance, including points, boxes, and coarse-grained masks; b) Unlike traditional image segmentation tasks, image manipulation detection tasks rely significantly on the guidance of semantic-agnostic information. In response to these challenges, this paper develops an image manipulation detection method, IMDPrompter, based on the foundational SAM model and incorporating various semantic-agnostic noise map information. Inspired by prompt learning, our IMDPrompter no longer depends on manual guidance but can achieve automated prompt learning. Moreover, we introduce components such as Semantic-Agnostic Feature Fusion (SAF), Optimal Prompt Selection (OPS), Cross-View Prompt Consistency (CPC), and Prompt Mixing Module (PMM), which fully integrate various semantic-agnostic information, enabling SAM to generate accurate tampered area masks for image manipulation detection. Extensive experimental results from the five datasets CASIA, Columbia, Coverage, IMD2020, and NIST16 validate the effectiveness of our proposed method.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}\label{sec:intro}
With the continuous emergence of powerful editing tools, manipulating images has become unprecedentedly simple. These new opportunities have sparked creativity among both benevolent and malevolent users. Previously, orchestrating multimedia disinformation campaigns required complex skills, and attackers could only splice, copy, or delete objects. With the explosive growth of deep learning, image editing tools have become more user-friendly and potent, allowing users to generate instant images of non-existent individuals or achieve convincing deepfakes. Generative models can produce realistic image edits using natural language prompts, seamlessly integrating inserted elements to match the style and lighting of the environment \cite{avrahami2023blended, nichol2021glide}.

The risks posed by these tools falling into the wrong hands are evident. In fact, in recent years, governments and funding agencies have shown increasing interest in developing forensic tools capable of addressing such attacks. The primary focus is on local image manipulation, particularly alterations that change the semantic content of images. To tackle these challenges, activities in the fields of multimedia forensics and related sciences have rapidly expanded, proposing numerous methods and tools for image manipulation detection and localization \cite{verdoliva2020media,cozzolino2022data,huh2018fighting,wu2019mantra}. Despite considerable progress in this field, the performance of current state-of-the-art detectors is insufficient for field deployment, primarily due to several shortcomings that require further research: i) limited generalizability; ii) limited robustness; and iii) inadequate detection performance.
\begin{figure}[t]
	\centering
	\includegraphics[width=0.7\linewidth]{sec/fig/intro.pdf}
	\caption{Improvements of IMDPrompter over baseline methods: a.Automated prompt learning without the need for manual input; b.Integration of semantic-agnostic information crucial for Image Manipulation Detection.}
	\label{fig:intro}
\end{figure}

To address the shortcomings of existing image manipulation detection methods, we turn our attention to foundational models. Benefiting from large-scale pretraining, foundational models such as GPT-4 \cite{achiam2023gpt}, Flamingo \cite{alayrac2022flamingo}, and SAM \cite{kirillov2023segment} have made significant advancements and contributed greatly to societal progress. Among these, SAM, trained on 1 billion masks, and demonstrating outstanding generalization capabilities, has inspired our research. However, SAM's interactive framework requires pre-provided cues such as points, boxes, or masks alongside input images. Operating as a category-agnostic segmentation method, as shown in Figure 1, these limitations render SAM unsuitable for fully automated understanding in image manipulation detection. Furthermore, we note that unlike previous tasks like semantic or instance segmentation, image manipulation detection methods require the introduction of semantic-agnostic features; relying solely on RGB visual features is insufficient to address image manipulation detection problems  \cite{chen2021image}, posing significant challenges for SAM in image manipulation detection work.


To enhance the image manipulation detection capabilities of foundational models, we propose a new method called IMDPrompter for learning how to generate prompts that enhance the functionality of the SAM framework. Our research primarily focuses on the SAM framework, which is a category-agnostic interactive segmentation model. To introduce semantic-agnostic features, we incorporate three noise views, SRM Filter \cite{zhou2018learning}, Bayer Conv \cite{bayar2018constrained}  and Noiseprint \cite{cozzolino2019noiseprint}. For integrating RGB visual features with semantic-agnostic features, we build the Semantic-Agnostic Feature Fusion (SAF) module. For RGB views and three noise views, we sequentially acquire image manipulation localization masks. Additionally, we construct an ensemble mask outputting from four branches for selecting the optimal localization map to generate prompts, we construct the Optimal Prompt Selection (OPS) module based on minimizing localization loss. After obtaining the optimal prompt, to achieve cross-view prompt consistency enhancement, we introduce the Cross-View Prompt Consistency (CPC) loss constraint, aligning the localization maps of the four branches to the optimal localization map. Prompt Mixing Module is proposed to integrate multiple types of prompt information.

In summary, the main contributions are listed as follows.
\begin{itemize}
    \item We propose a learning paradigm called IMDPrompter for utilizing SAM in image manipulation detection, marking the first attempt to apply SAM to this field.
    \item We introduce an automated prompt learning method, which eliminates the need for manual guidance and simplifies the implementation of IMDPrompter.
    \item We develop components such as Semantic-Agnostic Feature Fusion, Optimal Prompt Selection, Cross-View Prompt Consistency, and Prompt Mixing Module to fully integrate various semantic-agnostic information.
    \item We demonstrate extensive results across five different image manipulation detection datasets, thoroughly validating the strong in-distribution and out-of-distribution image manipulation detection and localization capabilities of IMDPrompter.
\end{itemize}


% \begin{itemize}
%     \item 
%     We propose a method for learning prompts that incorporate semantic-agnostic information, enhancing the capability of the SAM model for image manipulation detection.
        
%     \item
%     We introduce methods such as Optimal Prompt Selection and Cross-View Prompt Consistency Enhancement to achieve optimized prompts and enhance cross-view consistency.
    
%     \item  
%     We propose a Prompt Mixing module to integrate prompts of multiple types.

%     \item  We demonstrate extensive results on five different image manipulation detection datasets, fully validating IMDPrompter's strong capabilities for in-distribution and out-of-distribution image manipulation detection and localization.
% \end{itemize}



==> sec/2_related_work.tex <==
\section{Related Work}

\noindent\textbf{Image Manipulation Detection.} Currently, methods for image manipulation detection can be broadly categorized into two types, primarily distinguished by their recognition of manipulated artifacts. Some techniques \cite{wu2019mantra, chen2021image, wu2022robust, bi2019rru, hu2020span, yang2020constrained, marra2020full} rely on detecting abnormal features and often use high-pass noise filters \cite{yang2020constrained, li2019localization} to suppress content information. Other methods \cite{park2018double, kwon2022learning, mareen2022comprint} attempt to detect inconsistencies in compression within tampered images, as they assume different compression Quality Factors (QFs) before and after the operation. Additionally, some researchers focus their attention on camera-based artifacts, such as model fingerprints \cite{mareen2022comprint, cozzolino2019noiseprint, cozzolino2015splicebuster}.

\noindent\textbf{Foundational Models.} In recent years, foundational models have sparked a tremendous transformation in the field of artificial intelligence. These models, trained on extensive datasets, have demonstrated impressive zero-shot generalization capabilities across various scenarios \cite{kirillov2023segment, radford2021learning, jia2021scaling, sharif2014cnn}. Renowned models such as Chat-GPT \cite{ouyang2022training}, GPT-4 \cite{achiam2023gpt}, and Stable Diffusion \cite{rombach2022high} have further propelled the development of artificial intelligence, making significant contributions to human civilization and exerting considerable influence across various industries. 
Inspired by the success of foundational models in natural language processing (NLP), researchers have begun exploring their potential applications in computer vision. While most of these models are aimed at extracting accessible knowledge from freely available data \cite{alayrac2022flamingo, radford2021learning, chen2023ovarnet}, the recent SAM model \cite{kirillov2023segment} adopts an innovative approach by constructing a data engine where the model co-develops annotations with environmental datasets. SAM uniquely leverages a vast collection of masks, showcasing robust generalization capabilities. However, it was initially designed as a task-agnostic segmentation model, requiring prompts (i.e., inputs of prior points, bounding boxes, or masks), and therefore does not directly facilitate end-to-end automated segmentation perception.
This paper does not delve into the design and training of foundational image manipulation detection models; instead, we explore the potential of utilizing SAM's powerful universal segmentation capabilities for image manipulation detection and localization. Furthermore, the proposed method of learning prompts can be extended to other visual foundational models beyond SAM.

\noindent\textbf{Prompt Learning.} In the past, machine learning tasks were primarily focused on fully supervised learning, where task-specific models were trained only on labeled instances of the target task  \cite{krizhevsky2017imagenet}. However, over time, there has been a significant shift in learning paradigms, transitioning from fully supervised learning towards \textit{pretraining and fine-tuning }approaches for downstream tasks. This shift allows models to leverage general features acquired during pretraining \cite{russakovsky2015imagenet, simonyan2014very, he2016deep}.
More recently, with the advent of foundational models, a new paradigm has emerged known as \textit{pretraining and prompting} \cite{chen2023ovarnet, lester2021power, liu2023pre, zhou2022learning}. In this paradigm, researchers no longer train models specifically for downstream tasks but instead redesign inputs using prompts to reformulate the downstream tasks to align with the original pretraining task \cite{radford2021learning, devlin2018bert, radford2019language}. Prompting helps to reduce semantic gaps, bridge the gap between pretraining and fine-tuning, and prevent overfitting of the heads. Since the advent of GPT-3 \cite{brown2020language}, prompting has evolved from traditional discrete \cite{liu2023pre} and continuous prompt constructions \cite{chen2023ovarnet, zhou2022learning} to large-scale model-centric contextual learning \cite{alayrac2022flamingo}, instruction tuning \cite{liu2024visual, peng2023instruction, gupta2022instructdial}, and chaining approaches \cite{wei2022chain, wang2022self, zhang2022automatic}.
Currently, methods for constructing prompts include manual templates, heuristic-based templates, generation, fine-tuning word embeddings, and pseudo-labeling \cite{liu2023pre, wang2022learning}. In this paper, we propose a prompt generator for generating prompts compatible with SAM.



==> sec/3_method.tex <==
\begin{figure*}[ht]
	\centering
	\includegraphics[width=\linewidth]{sec/fig/Pipeline.pdf}
	\caption{Overall framework of IMDPrompter. The prompter part consists of four views: RGB, SRM, Bayar and Noiseprint. OPS selects the optimal prediction from the four views to generate the best prompt. CPC enhances cross-view consistency. SAF introduces semantic-agnostic features. PMM achieves a mixture of multiple prompt information.}
	\label{fig:pipe}
\end{figure*}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.7\linewidth]{sec/fig/sae.pdf}
	\caption{Architecture of the Semantic-Agnostic Feature Fusion (SAF) unit.}
	\label{fig:saf}
\end{figure}
\section{Method}
As shown in Figure \ref{fig:pipe}, We achieve integration of information from the RGB view and three noise views, facilitating the automation of SAM prompts. Specifically, through the SAF module, we integrate the information from the noise views into the RGB view; through the optimal prompt selection module, we select the best prompts from multiple sparse prompts; via CPC, we enhance consistency across multiple views; and through the PMM module, we organize a mix of various types of prompts, achieving efficient, automated image manipulation detection and localization based on SAM.


\subsection{Semantic-Agnostic Feature Fusion}
Current technology finds that exploring semantic information from images works well for in-domain (IND) manipulation detection but performs poorly in out-of-domain (OOD) detection. Additionally, utilizing image noise maps to learn semantic-agnostic information can yield strong performance. Given these findings, we hypothesize that relying solely on semantically related information is insufficient for detecting and localizing manipulations. To address this issue, we introduce information from three semantic-agnostic views, the SRM noise map, the Bayer noise map, and the Noiseprint  noise map, with the process as follows:
\begin{equation}
F_{\text{sam}} = \Phi_{\text{sam-img}}(\mathcal{I})
\end{equation}
\begin{equation}
f_{\text{RGB}} = \Phi_{\text{Seg-RGB}}(\mathcal{I})
\end{equation}
\begin{equation}
f_{\text{SRM}} = \Phi_{\text{Seg-SRM}}\left(\Phi_{\text{SRM}}(\mathcal{I})\right)
\end{equation}
\begin{equation}
f_{\text{Bayer}} = \Phi_{\text{Seg-Bayer}}\left(\Phi_{\text{Bayer}}(\mathcal{I})\right)
\end{equation}
\begin{equation}
f_{\text{Noiseprint}} = \Phi_{\text{Seg-Noiseprint}}\left(\Phi_{\text{Noiseprint}}(\mathcal{I})\right)
\end{equation}
\begin{equation}
F_{\text{SAF}} = \Phi_{\text{SAF}}\left(F_{\text{sam}}, f_{\text{RGB}}, f_{\text{SRM}}, f_{\text{Bayer}},f_{\text{Noiseprint}}\right)
\end{equation}
In the system, $\mathcal{I}$ represents the input image, and $\Phi_{\text{sam-img}}$ denotes the SAM image encoder. $F_{\text{sam}}$ represents the features encoded by the SAM image encoder. $\Phi_{\mathrm{SRM}}$, $\Phi_{\text{Bayer}}$ and $\Phi_{\text{Noiseprint}}$ respectively represent the SRM noise map extractor, the Bayer noise map extractor and the Noiseprint noise map extractor. $\Phi_{\text{Seg-RGB}}$, $\Phi_{\text{Seg-SRM}}$, $\Phi_{\text{Seg-Bayer}}$ and $\Phi_{\text{Seg-Noiseprint}}$ each represent the segmenter for the RGB view, SRM view, Bayer view and Noiseprint view, with all four segmenters having identical structures but non-shared parameters. $f_{\mathrm{RGB}}$, $f_{\mathrm{SRM}}$, $f_{\mathrm{Bayer}}$ and $f_{\mathrm{Noiseprint}}$ represent the features from the RGB, SRM, Bayer, and Noiseprint views, respectively. $\Phi_{\mathrm{SAF}}$ stands for the module that integrates semantic-agnostic features, and $F_{\mathrm{SAF}}$ represents the fused features after integration by SAF. The structure diagram of the SAF module is shown in Figure \ref{fig:saf}.

Existing technology has shown that exploring semantic information from images is effective for in-domain (IND) manipulation detection but performs poorly in out-of-domain (OOD) detection. Additionally, utilizing noise maps from images to learn semantic-agnostic information can yield significant performance gains. Given these findings, we hypothesize that relying solely on semantically related information is insufficient for detecting and locating manipulations. To address this issue, we have incorporated information from two semantic-agnostic views, the SRM noise map ,the Bayer noise map and Noiseprint noise map. The entire process is illustrated in Figure \ref{fig:saf}.

First, the features $f_{\text{RGB}}$, $f_{\text{SRM}}$, $f_{\text{Bayer}}$, and $f_{\text{Noiseprint}}$ are aligned with $F_{\text{sam}}$ through bicubic interpolation, followed by channel concatenation with $F_{\text{sam}}$ after passing through a $1 \times 1$ convolution. The concatenated features then pass through two stacked convolution blocks (comprising $3 \times 3$ convolution, instance normalization, and GELU activation), and the output from the semantic selection attention branch (consisting of global average pooling, a fully connected layer, GELU, and sigmoid) is weighted onto the shortcut branch to produce the integrated feature $F_{\text{SAF}}$. Through the SAF module, features from multiple views are effectively integrated.

\subsection{Optimal Prompt Selection}
In the process of generating masked prompts, we utilize the mask probability distributions from four views, $P_{\mathrm{RGB}}$, $P_{\mathrm{SRM}}$, $P_{\mathrm{Bayar}}$, and $P_{\mathrm{Noiseprint}}$, and construct an integrated mask probability distribution $P_{\text{Ens}}$. We then select the optimal mask probability segmentation $P_{\mathrm{opt}}$ based on the principle of minimizing segmentation loss. Further, we obtain the mask $M_{\mathrm{opt}}$ and bounding box prompts $\mathcal{B}_{\mathrm{opt}}$, which are input into SAM's prompt encoder to obtain the prompt encoding $F_{\mathrm{opt}}$. The process is as follows:
\begin{equation}
P_{\mathrm{RGB}} = \Phi_{\mathrm{RGB}-\mathrm{CLS}}(f_{\mathrm{RGB}}),
\end{equation}
\begin{equation}
P_{\mathrm{SRM}} = \Phi_{\mathrm{SRM-CLS}}(f_{\mathrm{SRM}}),
\end{equation}
\begin{equation}
P_{\mathrm{Bayer}} = \Phi_{\mathrm{Bayer-CLS}}(f_{\mathrm{Bayer}}),
\end{equation}
\begin{equation}
P_{\mathrm{Noiseprint}} = \Phi_{\mathrm{Noiseprint-CLS}}(f_{\mathrm{Noiseprint}}),
\end{equation}
\begin{equation}
P_{\text{Ens}} = \frac{P_{\mathrm{RGB}} + P_{\mathrm{SRM}} + P_{\mathrm{Bayer}}+P_{\mathrm{Noiseprint}}}{4},
\end{equation}
\begin{equation}
\mathcal{P}=\{P_{\mathrm{RGB}}, P_{\mathrm{SRM}}, P_{\mathrm{Bayer}},P_{\mathrm{Noiseprint}}, P_{\text{Ens}}\},
\end{equation}
\begin{equation}
P_{\text{opt}} = \underset{P \in \mathcal{P}}{\operatorname{argmin}} L_{\mathrm{Seg}}(P, G),
\end{equation}
\begin{equation}
M_{\mathrm{opt}} = \Phi_{\mathrm{mask}}(P_{\mathrm{opt}}),
\end{equation}
\begin{equation}
\mathcal{B}_{\mathrm{opt}} = \Phi_{\mathrm{box}}(M_{\mathrm{opt}}),
\end{equation}
\begin{equation}
F_{\mathrm{opt}} = \Phi_{\mathrm{p-enc}}(M_{\mathrm{opt}}, \mathcal{B}_{\mathrm{opt}}),
\end{equation}
where $\Phi_{\mathrm{RGB-CLS}}$, $\Phi_{\mathrm{SRM-CLS}}$, $\Phi_{\mathrm{Bayer-CLS}}$ and $\Phi_{\mathrm{Noiseprint-CLS}}$ represent classifiers for the RGB, SRM, Bayer, and Noiseprint views, respectively, $G$ represents the one-hot encoded mask labels, $L_{\mathrm{Seg}}$ is the segmentation loss function, $\Phi_{\mathrm{mask}}$ represents the mask generation operation, $\Phi_{\mathrm{box}}$ is the bounding box generation operation, and $\Phi_{\mathrm{p-enc}}$ represents SAM's prompt encoder.

\subsection{Cross-View Prompt Consistency}
Ideally, the segmentation masks from the four views should be consistent with the optimal segmentation mask. Therefore, we constructed a cross-view prompt consistency enhancement loss to achieve enhanced prompt consistency across views. The $\mathrm{CPC}$ loss function is expressed as follows:
\begin{equation}
\mathcal{L}_{\mathrm{CPC}} = \mathcal{L}_{\mathrm{Seg}}(P_{\mathrm{RGB}}, P_{\text{opt}}) + \mathcal{L}_{\mathrm{Seg}}(P_{\mathrm{SRM}}, P_{\text{opt}}) + \mathcal{L}_{\mathrm{Seg}}(P_{\mathrm{Bayer}}, P_{\text{opt}}) +
\mathcal{L}_{\mathrm{Seg}}(P_{\mathrm{Noiseprint}}, P_{\text{opt}})
\end{equation}

Where $\mathcal{L}_{\mathrm{Seg}}$ is the segmentation loss function.

\subsection{Prompt Mixing Module}
Since $F_{\mathrm{SAF}}$ aggregates semantically related and unrelated features, it aids the guidance of SAM for image manipulation detection. Therefore, we constructed the PMM module, which is primarily based on MLP, to integrate multiple types of prompt information. First, the two types of prompt inputs, $F_{\mathrm{SAF}}$ and $F_{\mathrm{opt}}$, are concatenated, followed by an MLP layer to perform dimension transformation to align with the original SAM prompt encoder's prompt embedding. Then, $F_{\mathrm{mix}}$ and $F_{\mathrm{SAF}}$ are input into SAM's mask decoder to achieve the image manipulation localization process. The process is as follows:
\begin{equation}
F_{\mathrm{mix}} = \Phi_{\mathrm{MLP}}\left([F_{\mathrm{SAF}} ; F_{\mathrm{opt}}]\right),
\end{equation}
\begin{equation}
P_{\mathrm{sam}} = \Phi_{\mathrm{sam-dec}}(F_{\mathrm{SAF}}, F_{\mathrm{mix}}),
\end{equation}
where $\Phi_{\mathrm{MLP}}$ represents the MLP layer operation, $F_{\mathrm{mix}}$ represents the integrated prompt embedding, and $\Phi_{\mathrm{sam-dec}}$ represents SAM's mask decoder, with $P_{\mathrm{sam}}$ representing the mask probability prediction output of the mask decoder.

\subsection{Training and Inference Pipeline}
The training loss function of IMDPrompter includes the segmentation loss from four prompt views $\mathcal{L}_{\text{Seg-p}}$, the CPC loss $\mathcal{L}_{\mathrm{CPC}}$, the SAM decoder segmentation loss $\mathcal{L}_{\text{Seg-sam}}$, and the image-level prediction loss $\mathcal{L}_{\text{Img-level}}$. The formula is expressed as follows:
\begin{equation}
\mathcal{L} = \mathcal{L}_{\text{Seg-sam}} + \lambda_1 \mathcal{L}_{\text{Seg-p}} + \lambda_2 \mathcal{L}_{\mathrm{CPC}} + \lambda_3 \mathcal{L}_{\text{Img-level}},
\end{equation}
where
\begin{equation}
L_{\text{Seg-sam}} = L_{\text{Seg}}(P_{\text{sam}}, G)
\end{equation}
\begin{equation}
L_{\text{Seg-p}} = L_{\text{Seg}}(P_{\text{RGB}}, G) + L_{\text{Seg}}(P_{\text{Bayar}}, G) + L_{\text{Seg}}(P_{\text{SRM}}, G)+ L_{\text{Seg}}(P_{\text{Noiseprint}}, G)
\end{equation}

In this paper, we use Focal Loss as our $L_{\mathrm{Seg}}$.

For image-level detection, following the work of \cite{zhai2023towards}, we adopt an adaptive pooling based on minimizing intra-class prediction variance. The overall computational process is as follows, first using Otsu's method \cite{otsu1975threshold} to find a threshold $\omega_0$ that minimizes the intra-class prediction variance:
\begin{equation}
\begin{array}{r}
\omega_0=\underset{\omega \in\left\{\hat{p}_{i, j}\right\}}{\arg \min }\left|\left\{\hat{p}_{i, j} \mid \hat{p}_{i, j}<\omega\right\}\right| \operatorname{var}\left(\left\{\hat{p}_{i, j} \mid \hat{p}_{i, j}<\omega\right\}\right)+ \\
\left|\left\{\hat{p}_{i, j} \mid \hat{p}_{i, j} \geq \omega\right\}\right| \operatorname{var}\left(\left\{\hat{p}_{i, j} \mid \hat{p}_{i, j} \geq \omega\right\}\right),
\end{array}
\end{equation}
where $\operatorname{var}(\cdot)$ denotes variance, $\hat{p}_{i, j}$ is the pixel-level response at position $(i, j)$.
Then the image-level prediction is aggregated from pixel-level responses above the threshold and the image-level loss is:
\begin{equation}
\hat{y}_{\mathrm{A}} = \frac{1}{\left| \mathbb{P}_{\mathrm{h}} \right|} \sum_{\hat{p} \in \mathbb{P}_{\mathrm{h}}} \hat{p}; \mathbb{P}_{\mathrm{h}} = \left\{\hat{p}_{i, j} \mid \hat{p}_{i, j} \geq \omega_0\right\},
\end{equation}
\begin{equation}
\mathcal{L}_{\text{Img-level}} = \mathcal{L}_{\mathrm{BCE}}(y, \hat{y}_{\mathrm{A}}),
\end{equation}
where $\hat{y}_{\mathrm{A}}$ is the image-level prediction, $\mathcal{L}_{\mathrm{BCE}}$ denotes the binary cross-entropy loss.

During the inference process of IMDPrompter, since there are no true labels, our OPS module defaults to selecting $P_{\text{Ens}}$ for generating  masks and bounding box prompts, with other components functioning as during the training process.




==> sec/4_experiment.tex <==
\section{Experiment}
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\linewidth]{sec/fig/vis.pdf}
	\caption{ Visualization Comparison of Image Manipulation Detection and Localization Results}
	\label{vis}
\end{figure*}
\input{sec/table/4-1-1}
\input{sec/table/4-1-2}
\input{sec/table/4-1-3}



% \input{sec/table/new-3}
% \input{sec/table/new-4}



% % \input{sec/table/new-5}
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.80\textwidth, keepaspectratio]{sec/fig/combined_chart.pdf}
% 	\caption{Radar chart comparing experimental performance with mainstream methods.}
 
% 	\label{sensitivity}
% \end{figure}

% \begin{figure}[ht]
%     \centering
    
%     \begin{subfigure}{\columnwidth} 
%         \centering
%         \includegraphics[width=0.80\textwidth]{sec/fig/IMDP-111.pdf}  % Adjust the image width as necessary, here set to 75% of the column width
%         \caption{ Bar chart analysis of ablation experiments on the IND dataset.}
%         \label{fig:sub1}
%     \end{subfigure}
    
%     \vspace{0.3cm} 
%     \begin{subfigure}{\columnwidth}  
%         \centering
%         \includegraphics[width=0.80\textwidth]{sec/fig/IMDP-222.pdf}
%         \caption{ Bar chart analysis of ablation experiments on the OOD dataset.}
%         \label{fig:sub2}
%     \end{subfigure}
    
%     \caption{Bar chart analysis of ablation experiments.}
%     \label{fig:test}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{sec/fig/IMDP-111.pdf}
%         \caption{ Bar chart analysis of ablation experiments on the IND dataset.}
%         \label{fig:sub1}
%     \end{minipage}\hfill
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{sec/fig/IMDP-222.pdf}
%         \caption{ Bar chart analysis of ablation experiments on the OOD dataset.}
%         \label{fig:sub2}
%     \end{minipage}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}  % 
%         \centering
%         \includegraphics[width=\textwidth]{sec/fig/IMDP-111.pdf}  % 
%         \caption{Bar chart analysis of ablation experiments on the IND dataset.}
%         \label{fig:sub1}
%     \end{subfigure}
%     \hfill  %
%     \begin{subfigure}[b]{0.49\textwidth}  % 
%         \centering
%         \includegraphics[width=\textwidth]{sec/fig/IMDP-222.pdf}
%         \caption{Bar chart analysis of ablation experiments on the OOD dataset.}
%         \label{fig:sub2}
%     \end{subfigure}
%     \caption{Bar chart analysis of ablation experiments.}
%     \label{fig:test}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     % First row
%     \begin{subfigure}{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{sec/fig/IMDP-rada-1-F1}
%         \caption{ I-F1 radar chart}
%         \label{fig:sub1}
%     \end{subfigure}
%     \hfill  
%     \begin{subfigure}{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{sec/fig/IMDP-rada-1-AUC}
%         \caption{I-AUC radar chart}
%         \label{fig:sub3}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{sec/fig/IMDP-rada-2}
%         \caption{Com-F1 radar chart}
%         \label{fig:sub4}
%     \end{subfigure}

%     % Third row
%     \begin{subfigure}{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{sec/fig/IMDP-rada-3-1}
%         \caption{Best threshold P-F1 radar chart}
%         \label{fig:sub5}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{sec/fig/IMDP-rada-3-2}
%         \caption{Fixed threshold P-F1 radar chart}
%         \label{fig:sub6}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.3\columnwidth}
%         \centering
%         \includegraphics[width=\linewidth]{sec/fig/radar_chart_legend.pdf}
%         \caption{ }
%         \label{fig:sub2}
%     \end{subfigure}
    
%     \caption{Radar chart comparing experimental performance with mainstream methods.}
%     \label{fig:grid}
% \end{figure}





\noindent\textbf{Dataset.} Our method is trained only on the CASIAv2 dataset \cite{dong2013casia}. For in-distribution (IND) evaluation, we use the CASIAv1 dataset \cite{dong2013casia}. For out-of-distribution (OOD) evaluation, we use three datasets: Columbia \cite{hsu2006detecting}, Coverage \cite{wen2016coverage}and IMD2020 \cite{novozamsky2020imd2020}. 

\noindent\textbf{Evaluation Metrics.} For image-level manipulation detection, we report specificity, sensitivity, and their F1-score (I-F1). The area under the receiver operating characteristic curve (AUC) is also reported as a threshold-independent metric for image-level detection. For pixel-level manipulation localization, we follow previous methods\cite{chen2021image,zhou2018learning,zhou2018generate,salloum2018image} to compute pixel accuracy, recall, and their F1-score (P-F1) on manipulated images. The overall performance of image and pixel-level manipulation detection/localization is measured by the harmonic mean of pixel-level and image-level F1-scores \cite{chen2021image}, denoted as composite F1 (Com-F1), and is sensitive to lower values of P-F1 and I-F1. To ensure fair comparison, a default threshold of 0.5 is used for F1 computation unless otherwise specified.

\noindent\textbf{Implementation Details.} In our experiments, unless otherwise specified, we consistently use the VIT-L backbone of SAM and employ FCN as the segmentor for the three prompt views. We maintain image size at 1024×1024, consistent with the original input of the SAM model. To augment training samples, we use data augmentation techniques such as horizontal flipping and random cropping. The image encoder remains frozen during the training phase. All experiments are run on NVIDIA A6000 GPUs. For the optimization process, we train our model using the AdamW optimizer with an initial learning rate of 1e-4. We use a batch size of 4 and train for 100 epochs. We implement a linear warm-up strategy with a cosine annealing scheduler \cite{loshchilov2016sgdr} to decay the learning rate. Our proposed method is developed using PyTorch.

\subsection{
Comparison with State-of-the-Art Method}

\noindent\textbf{Pixel-level Manipulation Detection}
Table \ref{4-1-1} illustrates the pixel-level detection performance of different models. We evaluate the F1-score under two settings: best threshold and fixed threshold (0.5). From Table \ref{4-1-1}, it is evident that IMDPrompter achieves the best performance across nearly all datasets. Under the optimal threshold setting, we achieved an average F1 Score of 81.36\%. Under the fixed threshold setting, IMDPrompter achieved an average F1 Score of 59.78\%, indicating that our proposed IMDPrompter demonstrates better robustness in threshold settings.

\noindent\textbf{Image-level Manipulation Detection.}
Table \ref{4-1-2} presents the image-level performance of different models. For image-level performance, we use a default decision threshold of 0.5. Once again, IMDPrompter emerges as the top performer, leveraging our prompt learning paradigm to achieve higher specificity in most test settings, thereby reducing false positives. Additionally, IMDPrompter achieves the best average AUC and average F1-scores. The average F1-score of IMDPrompter significantly surpasses that of the second-best method, MVSS-Net, with an improvement of 38.4\%.

% \noindent\textbf{Image-level Operation Detection.}
% Table \ref{4-1-3} provides the overall performance of pixel-level and image-level operation detection. We calculate the harmonic mean of image-level detection F1 and pixel-level localization F1, termed Com-F1, as our overall performance evaluation metric. As shown in Table VII, IMDPrompter achieves the best performance across all settings. In terms of average Com-F1-score, we achieve a performance gain of 24.8\% relative to the second-best method, particularly demonstrating a substantial performance gain of 77.6\% in experiments on the COVER dataset.


% \noindent\textbf{Performance of Detection and Localization Overall.} 
% Table VII presents the overall performance of pixel-level and image-level manipulation detection. We evaluate the overall performance by computing the harmonic mean of image-level detection F1 and pixel-level localization F1, denoted as Com-F1. As shown in Table III, IMDPrompter achieves the best performance across all settings, showing a performance gain of 24.8\% relative to the second-best method in terms of average Com-F1-score. Particularly in experiments with the COVER dataset, we achieve a performance gain of 77.6\%.

% \noindent\textbf{Qualitative Results.}

% \noindent\textbf{Robustness Evaluation.} Following\cite{bi2019rru,hu2020span,li2019localization}, we assess the robustness of the model under two common manipulation operations encountered when images are shared on the internet: JPEG compression and Gaussian blur. Comparing these two operations, Gaussian blur has a more significant impact on detection performance, especially when using larger 17×17 scale convolution kernels. Our IMDPrompter exhibits better robustness compared to previous methods under these conditions.

\subsection{Ablation Studies}
% \noindent % 确保内容从页面边缘开始

% \begin{minipage}[t]{0.48\textwidth} % 左侧半页
% \centering
% \captionof{table}{Evaluation of each component of our method in IND dataset.} % 使用 captionof 来为 minipage 中的表格添加标题
% \renewcommand\arraystretch{1.2}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|cccc|ccc}
% \hline
% \multirow{2}{*}{} & \multirow{2}{*}{SAF} & \multirow{2}{*}{CPC} & \multirow{2}{*}{OPS} & \multirow{2}{*}{PMM} & \multicolumn{3}{c}{CASIA} \\ \cline{6-8} 
%                   &                      &                      &                       &                      & I-F1   & P-F1   & Com-F1  \\ \hline
% \Rmnum{1}               &                      &                      &                       &                      & 70.6   & 44.6   & 54.7    \\
% \Rmnum{2}               & $\checkmark$         &                      &                       &                      & 73.2   & 47.2   & 57.4    \\
% \Rmnum{3}               & $\checkmark$         & $\checkmark$         &                       &                      & 74.3   & 48.3   & 58.5    \\
% \Rmnum{4}               & $\checkmark$         & $\checkmark$         & $\checkmark$          &                      & 75.1   & 50.4   & 60.3    \\
% \Rmnum{5}               & $\checkmark$         & $\checkmark$         & $\checkmark$          & $\checkmark$         & 77.3   & 50.6   & 61.2    \\ \hline
% \end{tabular}
% }
% \label{AS1}
% \end{minipage}%
% \hspace{0.3cm}  % 添加空格以隔开两个 minipage
% \begin{minipage}[t]{0.48\textwidth} % 右侧半页
% \centering
% \captionof{table}{Evaluation of each component of our method in OOD dataset.}
% \renewcommand\arraystretch{1.2}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|cccc|ccc}
% \hline
% \multirow{2}{*}{} & \multirow{2}{*}{SAF} & \multirow{2}{*}{CPC} & \multirow{2}{*}{OPS} & \multirow{2}{*}{PMM} & \multicolumn{3}{c}{COVER} \\ \cline{6-8} 
%                   &                      &                      &                       &                      & I-F1   & P-F1   & Com-F1  \\ \hline
% \Rmnum{6}         &                      &                      &                       &                      & 20.4   & 23.1   & 21.7    \\
% \Rmnum{7}         & $\checkmark$         &                      &                       &                      & 49.6   & 37.6   & 42.8    \\
% \Rmnum{8}         & $\checkmark$         & $\checkmark$         &                       &                      & 58.6   & 40.3   & 47.8    \\
% \Rmnum{9}         & $\checkmark$         & $\checkmark$         & $\checkmark$          &                      & 65.2   & 44.7   & 53.0    \\
% \Rmnum{10}        & $\checkmark$         & $\checkmark$         & $\checkmark$          & $\checkmark$         & 70.3   & 46.9   & 56.3    \\ \hline
% \end{tabular}
% }
% \label{AS2}
% \end{minipage}
\begin{minipage}[t]{0.48\textwidth} % 左侧半页
\centering
\captionof{table}{Evaluation of each component of our method in IND dataset.} % 使用 captionof 来为 minipage 中的表格添加标题
\renewcommand\arraystretch{1.2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc|ccc}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{SAF} & \multirow{2}{*}{CPC} & \multirow{2}{*}{OPS} & \multirow{2}{*}{PMM} & \multicolumn{3}{c}{CASIA} \\ \cline{6-8} 
                  &                      &                      &                       &                      & I-F1   & P-F1   & Com-F1  \\ \hline
\Rmnum{1}               &                      &                      &                       &                      & 70.6   & 70.3   & 70.4    \\
\Rmnum{2}               & $\checkmark$         &                      &                       &                      & 73.2   & 73.1   & 73.1    \\
\Rmnum{3}               & $\checkmark$         & $\checkmark$         &                       &                      & 74.3   & 74.3   & 74.3    \\
\Rmnum{4}               & $\checkmark$         & $\checkmark$         & $\checkmark$          &                      & 75.1   & 76.1   & 75.6    \\
\Rmnum{5}               & $\checkmark$         & $\checkmark$         & $\checkmark$          & $\checkmark$         & 77.3   & 76.3   & 76.8    \\ \hline
\end{tabular}
}
\label{AS1}
\end{minipage}%
\hspace{0.3cm}  % 添加空格以隔开两个 minipage
\begin{minipage}[t]{0.48\textwidth} % 右侧半页
\centering
\captionof{table}{Evaluation of each component of our method in OOD dataset.}
\renewcommand\arraystretch{1.2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|cccc|ccc}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{SAF} & \multirow{2}{*}{CPC} & \multirow{2}{*}{OPS} & \multirow{2}{*}{PMM} & \multicolumn{3}{c}{COVER} \\ \cline{6-8} 
                  &                      &                      &                       &                      & I-F1   & P-F1   & Com-F1  \\ \hline
\Rmnum{6}         &                      &                      &                       &                      & 20.4   & 39.8   & 27.0    \\
\Rmnum{7}         & $\checkmark$         &                      &                       &                      & 49.6   & 54.3   & 51.8    \\
\Rmnum{8}         & $\checkmark$         & $\checkmark$         &                       &                      & 58.6   & 57.0   & 57.8    \\
\Rmnum{9}         & $\checkmark$         & $\checkmark$         & $\checkmark$          &                      & 65.2   & 61.4   & 63.2    \\
\Rmnum{10}        & $\checkmark$         & $\checkmark$         & $\checkmark$          & $\checkmark$         & 70.3   & 63.6   & 66.8    \\ \hline
\end{tabular}
}
\label{AS2}
\end{minipage}

To reveal the impact of different components, we evaluated the proposed model under different settings, incrementally adding components and considering the distinct impacts of each component on in-domain and out-of-domain datasets. Thus, we conducted ablation experiments on two test sets, CASIA and COVER, for in-domain and out-of-domain data, respectively, as shown  in Tables \ref{AS1} and \ref{AS2}.

\noindent\textbf{Baseline.}  From \textit{Experiment \Rmnum{1}}, it is known that our baseline method achieved performance scores of 70.6\%, 70.3\%, and 70.4\% on the I-F1, P-F1, and Com-F1 metrics respectively in the CASIA dataset. In the COVER dataset, it scored 20.4\%, 39.8\%, and 27.0\% on the same metrics. These experiments show that using only RGB visual view information has limited generalization ability in out-of-domain datasets.

\noindent\textbf{Impact of SAF.} From \textit{Experiment \Rmnum{2}}, with the addition of SAF which introduced semantically unrelated view information, there was an increase in performance on the CASIA dataset's I-F1, P-F1, Com-F1 metrics by 2.6\%, 2.8\%, and 2.7\% respectively. Experiment VII showed that on the COVER dataset, there was a performance gain of 29.2\%, 14.5\%, and 24.8\% respectively on the I-F1, P-F1, Com-F1 metrics, indicating that introducing semantically unrelated information can enhance performance in both in-domain and out-of-domain datasets, especially in the in-domain datasets.

\noindent\textbf{Impact of CPC.} From \textit{Experiment \Rmnum{3}}, the inclusion of CPC, which introduced cross-view consistency enhancement, resulted in performance gains of 3.7\%, 4.0\%, and 3.9\% on the I-F1, P-F1, Com-F1 metrics respectively in the CASIA dataset. Experiment VIII showed performance gains of 38.2\%, 17.2\%, and 30.8\% respectively on the COVER dataset, confirming that the prompt information between different views is complementary and integrative enhancement can bring objective performance improvements.

\noindent\textbf{Impact of OPS.} From \textit{Experiment \Rmnum{4}}, the inclusion of CPC adaptive selection of the optimal prompts resulted in performance gains of 4.5\%, 5.8\%, and 5.2\% on the I-F1, P-F1, Com-F1 metrics respectively in the CASIA dataset. Experiment IX showed gains of 44.8\%, 21.6\%, and 36.2\% respectively on the COVER dataset, indicating that simply adding together prompts from different views is not enough to generate the best prompts, and a optimal prompts selection strategy can optimize the prompt selection process.

\noindent\textbf{Impact of PMM.} From \textit{Experiment \Rmnum{5}}, with the inclusion of PMM which fully integrates various types of prompt information, there was an increase in performance of 6.7\%, 6.0\%, and 6.4\% on the I-F1, P-F1, Com-F1 metrics respectively in the CASIA dataset. \textit{Experiment \Rmnum{10}} showed an increase of 49.9\%, 23.8\%, and 39.8\% respectively on the COVER dataset, further demonstrating the effectiveness of PMM.















==> sec/5_conclusion.tex <==
\section{Conslusion}
In this paper, we propose a novel image manipulation detection prompt learning method, IMDPrompter, utilizing the SAM foundational model. The primary goal of IMDPrompter is to learn the generation of SAM prompt inputs, thereby automating image manipulation detection and localization tasks. Considering the reliance of image manipulation detection on semantically unrelated information, we constructed an integration and enhancement framework that merges multiple types of view information to achieve optimal prompt selection and mixing. We introduced modules such as SAF, CPC, OPS, and PMM to realize efficient image manipulation detection performance. Our IMDPrompter achieves objective image-level and pixel-level image manipulation detection performance in in-domain (IND) and out-of-domain (OOD) as well as various robustness evaluation settings.







==> sec/table/1-4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\caption{}
\centering
\resizebox{\textwidth}{!}{
\label{tab:my-table-4}
\begin{tabular}{@{}cccccccccccccccccll@{}}
\toprule
\multirow{2}{*}{} &
  \multicolumn{4}{c}{\textbf{CASIA}} &
  \multicolumn{4}{c}{\textbf{COVER}} &
  \multicolumn{4}{c}{\textbf{Columbia}} &
  \multicolumn{4}{c}{\textbf{IMD}} &
   &
   \\
   \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
 &
  \textbf{I-AUC} &
  \textbf{I-F1} &
  \textbf{P-F1} &
  \textbf{C-F1} &
  \textbf{I-AUC} &
  \textbf{I-F1} &
  \textbf{P-F1} &
  \textbf{C-F1} &
  \textbf{I-AUC} &
  \textbf{I-F1} &
  \textbf{P-F1} &
  \textbf{C-F1} &
  \textbf{I-AUC} &
  \textbf{I-F1} &
  \textbf{P-F1} &
  \textbf{C-F1} &
   &
   \\
   \cmidrule{2-17}
\textbf{MVSSNet\cite{chen2021image}}     & 0.937 & 75.8 & 45.2 & 56.6 & 0.731 & 24.4 & 45.3 & 31.7 & 0.980 & 80.2 & 63.8 & 71.1 & 0.656 & 35.5 & 26.0 & 30.0 &  &  \\
\textbf{Trufor\cite{guillaro2023trufor}}      & 0.916 & -    & 44.1 & -    & 0.770 & -    & 19.9 & -    & 0.996 & -    & 22.3 & -    & -     & -    & 21.0 & -    &  &  \\
\textbf{UNet\cite{ronneberger2015u}}        & 0.713 & 62.3 & 40.1 & 48.8 & 0.533 & 16.7 & 19.1 & 17.8 & 0.744 & 44.3 & 19.9 & 27.5 & 0.499 & 25.1 & 19.7 & 22.1 &  &  \\
\textbf{UNet+}       & 0.861 & 72.6 & 62.4 & 67.1 & 0.669 & 46.3 & 41.6 & 43.8 & 0.853 & 71.3 & 53.9 & 61.4 & 0.577 & 40.9 & 23.6 & 29.9 &  &  \\
\textbf{FCN\cite{long2015fully}}         & 0.770 & 68.3 & 44.1 & 53.6 & 0.541 & 18.0 & 19.9 & 18.9 & 0.762 & 48.1 & 22.3 & 30.5 & 0.502 & 26.2 & 21.0 & 23.3 &  &  \\
\textbf{FCN+}        & 0.873 & 73.4 & 61.3 & 66.8 & 0.681 & 49.2 & 43.9 & 46.4 & 0.871 & 72.6 & 52.4 & 60.9 & 0.589 & 43.1 & 25.1 & 31.7 &  &  \\
\textbf{IMDPrompter} & 0.978 & 77.3 & 76.3 & 76.8 & 0.796 & 70.3 & 63.6 & 66.8 & 0.983 & 93.6 & 87.3 & 90.3 & 0.671 & 63.7 & 30.6 & 41.3 & \\ \bottomrule
\end{tabular}
}
\end{table}

==> sec/table/baseline-on_THUMOS14.tex <==
\iffalse
\begin{table*}[htb]
\centering
\renewcommand\arraystretch{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccccc}
\hline
\multirow{2}{*}{\textbf{Supervision}}& \multirow{2}{*}{\textbf{Method}}& \multirow{2}{*}{\textbf{Publication}}& \multicolumn{6}{c}{\textbf{mAP@IoU}} \\
\cline{4-9}
&&& 0.3& 0.4& 0.5& 0.6& 0.7& AVG\\ \hline
\multirow{3}{*}{Fully}& DBS& \textit{AAAI 19}& 50.6& 43.1& 34.3& 24.4& 14.7& 33.4  \\
& BMN& \textit{ICCV 19}& 56& 47.4& 38.8& 29.7& 20.5& 38.5  \\
& BUMR& \textit{ECCV 20}& 53.9& 50.7& 45.4& 38& 28.5& 43.3  \\
\hline
\multirow{19}{*}{Weakly}& HAM-Net& \textit{AAAI 21}& 50.3& 41.1& 31& 20.7& 11.4& 30.9  \\
& UM& \textit{AAAI 21}& 49& 40.9& 30.4& 21& 10.4& 30.3  \\
& TS-PCA& \textit{CVPR 21}& 53.4& 43.4& 34.3& 24.7& 13.7& 33.9  \\
& CO$_2$-Net& \textit{MM 21}& 54.5& 45.7& 38.3& 26.4& 13.4& 35.7  \\
& ACM-Net& \textit{TIP 21}& 55.0& 44.6& 34.6& 21.8& 10.8& 33.4 \\
& FTCL& \textit{CVPR 22}& 55.2& 45.2& 35.6& 23.7& 12.2& 34.4  \\
& ACGNet& \textit{AAAI 22}& 53.1& 44.6& 34.7& 22.6& 12& 33.4  \\
& DCC& \textit{CVPR 22}& 55.9& 45.9& 35.7& 24.3& 13.7& 35.1  \\
& ASM-Loc& \textit{CVPR 22}& 57.1& 46.8& 36.6& 25.2& 13.4& 35.8  \\
& RSKP& \textit{CVPR 22}& 55.8& 47.5& 38.2& 25.4& 12.5& 35.9  \\
& DELU& \textit{ECCV 22}& 56.5& 47.7& 40.5& 27.2& 12.3& 37.4  \\
&ECM&\textit{TPAMI 22}& 46.5& 38.2& 29.1& 19.5& 10.9& 28.84 \\
& TSN-SAM& \textit{CVPR 23}& 60& 47.9& 37.1& 24.4& 12.7& 36.4  \\
& P-MIL& \textit{CVPR 23}& 58.9& 49& 40& 27.1& 15.1& 38\\
& BTGPL& \textit{CVPR 23}& 60.7& 51.8& 42.7& 26.2& 13.1& 38.9  \\
& DVLP& \textit{CVPR 23}& 61.5& \textbf{53.8}& 42& 29.4& 16.8& 40.7  \\
& PivoTAL& \textit{CVPR 23}& \textbf{61.7}& 52.1& \textbf{42.8}& 30.6& 16.7& 40.8  \\
& CASE& \textit{ICCV 23}& 59.2&& 37.7&& 13.7&\\
& AHLM& \textit{ICCV 23}& 60.2& 48.9& 38.3& 26.8& 14.7& 37.78 \\
& DDG-Net& \textit{ICCV 23}& 56.5& 47.7& 40.5& 27.2& 15.3& 37.44 \\ 
& BRD& \textit{TPAMI 23}& 58.3& 48.8& 36.5& 24.4& 13.4& 36.3 \\
\cline{2-9} 
& \textbf{NoCo (Ours)}&& 58.4& 51.5& 42.3& \textbf{32.8}& \textbf{22.7}& \textbf{41.5} \\
 \hline
\end{tabular}
}
\caption{Comparisons with state-of-the-art methods on THUMOS14 dataset. The average mAPs are computed under the IoU thresholds 0.3:0.1:0.7.}
\label{baseline-on THUMOS14}
\end{table*}
\fi

\iffalse
\begin{table*}[htp]
\centering
\renewcommand\arraystretch{1.1}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Supervision}}}& \multirow{2}{*}{\textbf{Method}}& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Publication}}}& \multicolumn{7}{c}{\textbf{mAP@IoU(\%)}}& \multicolumn{3}{c}{\textbf{AVG(\%)}}                       \\ \cline{4-13} 
\multicolumn{1}{c|}{}&& \multicolumn{1}{c|}{}& 0.1& 0.2& 0.3& 0.4& 0.5& 0.6& \multicolumn{1}{c|}{0.7}& 0.1:0.5& 0.3:0.7& 0.1:0.7  \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Fully}}& DBS& \multicolumn{1}{c|}{\textit{AAAI 2019}}& 56.7& 54.7& 50.6& 43.1& 34.3& 24.4& \multicolumn{1}{c|}{14.7}& 47.9& 33.4& 39.8  \\
\multicolumn{1}{c|}{}& BUMR& \multicolumn{1}{c|}{\textit{ECCV 2020}}& -& -& 53.9& 50.7& 45.4& 38& \multicolumn{1}{c|}{28.5}& -& 43.3& -  \\
\multicolumn{1}{c|}{}& BMN& \multicolumn{1}{c|}{\textit{ICCV 2019}}& -& -& 56& 47.4& 38.8& 29.7& \multicolumn{1}{c|}{20.5}& -& 38.5& -  \\ \hline
\multicolumn{1}{c|}{\multirow{18}{*}{Weakly}} 
%& HAM-Net& \multicolumn{1}{c|}{\textit{AAAI 2021}}& 65.4& 59& 50.3& 41.1& 31& 20.7& \multicolumn{1}{c|}{11.4}& 49.4& 30.9& 39.8  \\
& UM& \multicolumn{1}{c|}{\textit{AAAI 2021}}& 63& 56.6& 49& 40.9& 30.4& 21& \multicolumn{1}{c|}{10.4}& 48& 30.3& 38.8  \\
\multicolumn{1}{c|}{}& TS-PCA& \multicolumn{1}{c|}{\textit{CVPR 2021}}& 67.6& 61.1& 53.4& 43.4& 34.3& 24.7& \multicolumn{1}{c|}{13.7}& 52& 33.9& 42.6  \\
\multicolumn{1}{c|}{}& CO$_2$-Net& \multicolumn{1}{c|}{\textit{MM 21}}& 70.1& 63.6& 54.5& 45.7& 38.3& 26.4& \multicolumn{1}{c|}{13.4}& 54.4& 35.7& 44.6  \\
\multicolumn{1}{c|}{}& ECM& \multicolumn{1}{c|}{\textit{TPAMI 2022}}& 62.6& 55.1& 46.5& 38.2& 29.1& 19.5& \multicolumn{1}{c|}{10.9}& 46.3& 28.8& 37.4  \\
%\multicolumn{1}{c|}{}& FTCL& \multicolumn{1}{c|}{\textit{CVPR 2022}}& 69.6& 63.4& 55.2& 45.2& 35.6& 23.7& \multicolumn{1}{c|}{12.2}& 53.8& 34.4& 43.6  \\
%\multicolumn{1}{c|}{}& ACGNet& \multicolumn{1}{c|}{\textit{AAAI 2022}}& 68.1& 62.6& 53.1& 44.6& 34.7& 22.6& \multicolumn{1}{c|}{12}& 52.6& 33.4& 42.5  \\
%\multicolumn{1}{c|}{}& DCC& \multicolumn{1}{c|}{\textit{CVPR 2022}}& 69& 63.8& 55.9& 45.9& 35.7& 24.3& \multicolumn{1}{c|}{13.7}& 54.1& 35.1& 44 \\
\multicolumn{1}{c|}{}& ASM-Loc& \multicolumn{1}{c|}{\textit{CVPR 2022}}& 71.2& 65.5& 57.1& 46.8& 36.6& 25.2& \multicolumn{1}{c|}{13.4}& 55.4& 35.8& 45.1  \\
%\multicolumn{1}{c|}{}& RSKP& \multicolumn{1}{c|}{\textit{CVPR 2022}}& 71.3& 65.3& 55.8& 47.5& 38.2& 25.4& \multicolumn{1}{c|}{12.5}& 55.6& 35.9& 45.1  \\
\multicolumn{1}{c|}{}& DELU& \multicolumn{1}{c|}{\textit{ECCV 2022}}& 71.5& 66.2& 56.5& 47.7& 40.5& 27.2& \multicolumn{1}{c|}{12.3}& 56.5& 37.4& 46 \\
\multicolumn{1}{c|}{}& TSN-SAM& \multicolumn{1}{c|}{\textit{CVPR 2023}}& 73.0& 68.2& 60& 47.9& 37.1& 24.4& \multicolumn{1}{c|}{12.7}& 53.3& 36.4& 41.7  \\
\multicolumn{1}{c|}{}& P-MIL& \multicolumn{1}{c|}{\textit{CVPR 2023}}& 71.8& 67.5& 58.9& 49& 40& 27.1& \multicolumn{1}{c|}{15.1}& 57.4& 38& 47 \\
\multicolumn{1}{c|}{}& BTGPL& \multicolumn{1}{c|}{\textit{CVPR 2023}}& 74.0& 69.4& 60.7& 51.8& 42.7& 26.2& \multicolumn{1}{c|}{13.1}& 59.7& 38.9& 48.3  \\
\multicolumn{1}{c|}{}& DVLP& \multicolumn{1}{c|}{\textit{CVPR 2023}}& 73.5& 68.8& 61.5& 53.8& 42& 29.4& \multicolumn{1}{c|}{16.8}& 60& 40.7& 49.4  \\
\multicolumn{1}{c|}{}& PivoTAL& \multicolumn{1}{c|}{\textit{CVPR 2023}}& 74.1& 69.6& 61.7& 52.1& 42.8& 30.6& \multicolumn{1}{c|}{16.7}& 60.1& 40.8& 49.6  \\
\multicolumn{1}{c|}{}& BRD& \multicolumn{1}{c|}{\textit{TPAMI 2023}}& 73.1& 65.3& 58.3& 48.8& 36.5& 24.4& \multicolumn{1}{c|}{13.4}& 56.4& 36.3& 45.7  \\ \cline{2-13} 
\multicolumn{1}{c|}{}& \textbf{NoCo (Ours)}& \multicolumn{1}{c|}{}& \textbf{75.2}& \textbf{70.7}& \textbf{63.0}& \textbf{54.1}& \textbf{44}& \textbf{31.7}& \multicolumn{1}{c|}{\textbf{17.7}}& \textbf{61.4}& \textbf{43.2}& \textbf{50.9} \\ \hline
\end{tabular}
}
\caption{Comparisons with state-of-the-art methods on THUMOS14 dataset.}
\label{baseline-on THUMOS14}
\end{table*}
\fi

==> sec/table/baseline-on_activetyNet_v1.2.tex <==
\iffalse
\begin{table}[htb]
\centering
\renewcommand\arraystretch{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccc}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Supverised}}}& \multirow{2}{*}{\textbf{Method}}& \multirow{2}{*}{\textbf{Publication}}& \multicolumn{4}{c}{\textbf{mAP@IoU(\%)}} \\ \cline{4-7} 
\multicolumn{1}{l|}{}&&& 0.5& 0.75& 0.95& AVG     \\ \hline
Fully& SSN \cite{zhao2017temporal}& \textit{ICCV 2017}& 41.3& 27& 6.1& 26.6    \\ \hline
\multirow{12}{*}{Weakly}& CleanNet \cite{liu2019weakly}& \textit{ICCV 2019}& 37.1& 20.3& 5& 21.6    \\
& CMCS& \textit{CVPR 2019}& 36& 22& 5.6& 22.4    \\
& TSCN& \textit{ECCV 2020}& 37.6& 23.7& 5.7& 23.6    \\
& BasNet& \textit{AAAI 2020}& 38.5& 24.2& 5.6& 24.3    \\
& DGAM& \textit{CVPR 2020}& 41& 23.5& 5.3& 24.4    \\
& UM& \textit{AAAI 2021}& 41.2& 25.6& 6& 25.9    \\
& ACGNet& \textit{AAAI 2022}& 41.8& 26& 5.9& 26.1    \\
& D2-Net& \textit{ICCV 2021}& 42.3& 25.5& 5.8& 26      \\
& CO$_2$-Net& \textit{MM 2021}& 43.3& 26.3& 5.2& 26.4    \\
& DELU& \textit{ECCV 2022}& 44.2& 26.7& 5.4& 26.9    \\
& DVLP& \textit{CVPR 2023}& 48.3& 29.3& 6.1& 29.6    \\ \cline{2-7} 
& \textbf{NoCo (Ours) }&& 49.1& 30.5& 10.3& 30.7    \\ \hline 
\end{tabular}
}
\caption{Comparisons with state-of-the-art methods on ActivityNet v1.2 dataset. The average mAPs are computed under the IoU thresholds 0.5:0.05:0.95.}
\label{baseline-on activetyNet v1.2}
\end{table}
\fi

==> sec/table/compare_with_sota2.tex <==
\begin{table*}[htb]
\centering
\renewcommand\arraystretch{1.2}
\caption{Comparisons with state-of-the-art methods. AVG is the average mAP under the IoU thresholds 0.1:0.1:0.7 for THUMOS14 dataset and 0.5:0.05:0.95 for activityNet v1.2 and v1.3. '-' means that the corresponding results are nor reported in the original papers. The best results are bold. The baselines are underlined. Red highlight represents the performance improvement.}
\resizebox{\linewidth}{!}{





\begin{tabular}{lc|cccccccccccccccc}
\hline
\multirow{3}{*}{\textbf{Method}}& \multirow{3}{*}{\textbf{Publication}}& \multicolumn{16}{c}{\textbf{mAP@IoU(\%)}} \\ 
\cline{3-18} 
&& \multicolumn{8}{c|}{\textbf{THUMOS14}}& \multicolumn{4}{c|}{\textbf{ActivityNet v1.2}}& \multicolumn{4}{c}{\textbf{ActivityNet v1.3}}               \\ 
&& 0.1& 0.2& 0.3& 0.4& 0.5& 0.6& 0.7& \multicolumn{1}{c|}{AVG}& 0.5& 0.75& 0.95& \multicolumn{1}{c|}{AVG}& 0.5& 0.75& 0.95& AVG           \\ 
\hline
\multicolumn{2}{l|}{\textbf{Fully-supervised TAL}} &&&&&&&&\multicolumn{1}{c|}{}&&&&\multicolumn{1}{c|}{}& & & & \\
SSN \cite{zhao2017temporal}& ICCV 2017& 60.3& 56.2& 50.6& 40.8& 29.1& -& -& \multicolumn{1}{c|}{-}& 41.3& 27.0& 6.1& \multicolumn{1}{c|}{26.6}& 43.3& 28.7& 5.63& 28.2          \\
BSN \cite{lin2018bsn}& ECCV 2018& 53.5& 45.0& 36.9& 28.4& 20.0& -& -& \multicolumn{1}{c|}{-}& -& -& -& \multicolumn{1}{c|}{-}& 46.5& 30.0& 8.0& 30.0            \\
TAL-Net \cite{chao2018rethinking}& CVPR 2018& 59.8& 57.1& 53.2& 48.5& 42.8& 33.8& 20.8& \multicolumn{1}{c|}{45.1}& -& -& -& \multicolumn{1}{c|}{-}& 38.2& 18.3& 1.3& 20.2          \\ 
\hline
\multicolumn{2}{l|}{\textbf{Weakly-supervised TAL}} &&&&&&&&\multicolumn{1}{c|}{}&&&&\multicolumn{1}{c|}{}& & & & \\
MSA-Net \cite{yang2021multi}& TIP 2021& 65.6& 60.7& 52.3& 41.6& 29.7& 20.6& 10.1& \multicolumn{1}{c|}{40.8}& 43.4& 28.4& 5.6& \multicolumn{1}{c|}{25.7}& 37.3& 23.6& 5.9& 23.5          \\
AUMN \cite{luo2021action}& CVPR 2021& 66.2& 61.9& 54.9& 44.4& 33.3& 20.5& 9.0& \multicolumn{1}{c|}{41.5}& 42.0& 25.0& 5.6& \multicolumn{1}{c|}{25.6}& 38.3& 23.5& 5.2& 23.5          \\
ECM \cite{zhao2022equivalent}& TPAMI 2022& 62.6& 55.1& 46.5& 38.2& 29.1& 19.5& 10.9& \multicolumn{1}{c|}{37.4}& 41.0& 24.9& 6.5& \multicolumn{1}{c|}{25.5}& 36.7& 23.6& 5.9& 23.5          \\
Huang \textit{et.al} \cite{huang2022weakly}& CVPR 2022& 71.3& 65.3& 55.8& 47.5& 38.2& 25.4& 12.5& \multicolumn{1}{c|}{45.1}& -& -& -& \multicolumn{1}{c|}{-}& 40.6& 24.6& 5.9& 25.0          \\
DELU \cite{chen2022dual}& ECCV 2022& 71.5& 66.2& 56.5& 47.7& 40.5& 27.2& 12.3& \multicolumn{1}{c|}{46.0}& 44.2& 26.7& 5.4& \multicolumn{1}{c|}{26.9}& -& -& -& -             \\
Xu \textit{et.al} \cite{xu2023bilateral}& TPAMI 2023& 73.1& 66.9& 58.3& 48.8& 36.5& 24.4& 13.4& \multicolumn{1}{c|}{45.9}& -& -& -& \multicolumn{1}{c|}{-}& 41.2& 25.0& 6.5& 25.5          \\
AICL \cite{li2023actionness}& AAAI 2023& 73.1& 67.8& 58.2& 48.7& 36.9& 25.3& 14.9& \multicolumn{1}{c|}{46.4}& \textbf{49.6}& 29.1& 5.9& \multicolumn{1}{c|}{29.9}& 44.2& 27.4& 5.8& 27.6          \\
STCL-Net \cite{fu2023semantic}& TPAMI 2023& 72.7& 67.1& 58.2& 49.7& 41.8& 28.7& 16.0& \multicolumn{1}{c|}{47.8}& 44.0 & 26.1& 5.3& \multicolumn{1}{c|}{26.6}& 40.6& 24.0& 6.0& 24.7          \\
Zhou \textit{et.al} \cite{zhou2023improving}& CVPR 2023& 74.0& 69.4& 60.7& 51.8& 42.7& 26.2& 13.1& \multicolumn{1}{c|}{48.2}& -& -& -& \multicolumn{1}{c|}{-}& 43.4& 28.8& 9.9& 28.8          \\
DVLP \cite{ju2023distilling}& CVPR 2023& 73.5& 68.8& 61.5& 53.8& 42.0& 29.4& 16.8& \multicolumn{1}{c|}{49.4}& 48.3& 29.3& 6.1& \multicolumn{1}{c|}{29.6}& -& -& -& -             \\
PivoTAL \cite{rizve2023pivotal}& CVPR 2023& 74.1& 69.6& 61.7& 52.1& 42.8& 30.6& 16.7& \multicolumn{1}{c|}{49.6}& -& -& -& \multicolumn{1}{c|}{-}& 45.1& 28.2& 5.0& 28.1          \\ 
CASE \cite{liu2023revisiting}& ICCV 2023& 72.3& 67.1& 59.2& 49.4 & 37.7& 24.2 & 13.7& \multicolumn{1}{c|}{46.2}& 43.8& 27.2& 6.7& \multicolumn{1}{c|}{27.9}& 43.2& 26.2& 6.7& 26.8          \\
AHLM \cite{wang2023weakly}& ICCV 2023& 75.1& 68.9& 60.2& 48.9& 38.3& 26.8& 14.7& \multicolumn{1}{c|}{47.6}& -& -& -& \multicolumn{1}{c|}{-}& 42.3& 24.8& 6.9& 25.9          \\

% \cline{1-18} 
\hdashline[5pt/1pt]

\underline{\textbf{CO$_2$-Net \cite{hong2021cross}}} & \multicolumn{1}{c|}{MM 2021}& 70.1& 63.6& 54.5& 45.7& 38.3& 26.4& 13.4& \multicolumn{1}{c|}{44.6}& 43.3& 26.3& 5.2& \multicolumn{1}{c|}{26.4}& -& -& -& -             \\

\multicolumn{2}{l|}{\textbf{CO$_2$-Net + NoCo (Ours)} }& 74.6 & 70.3 & 63.0 & 53.9 & 44.0 & 31.7 & 17.4 & \multicolumn{1}{c|}{50.7 \textcolor{red}{(+6.1)}}& 48.9 & 30.0 & 6.6 & \multicolumn{1}{c|}{30.1 \textcolor{red}{(+3.7)}}& -& -& -& -             \\

\hdashline[5pt/1pt]

\underline{\textbf{ASM-Loc \cite{he2022asm}}} & \multicolumn{1}{c|}{CVPR 2022}& 71.2& 65.5& 57.1& 46.8& 36.6& 25.2& 13.4& \multicolumn{1}{c|}{45.1}& 43.4 & 26.6 & 5.3 & \multicolumn{1}{c|}{26.5}& 41.0& 24.9& 6.2& 25.1          \\

\multicolumn{2}{l|}{\textbf{ASM-Loc + NoCo (Ours)}}& \textbf{75.2}& \textbf{70.7}& \textbf{63.0}& \textbf{54.1}& \textbf{44.0}& \textbf{31.7}& \textbf{17.7}& \multicolumn{1}{c|}{\textbf{50.9} \textcolor{red}{(+5.8)}}& 49.1& \textbf{30.5}& \textbf{6.7}& \multicolumn{1}{c|}{\textbf{30.7} \textcolor{red}{(+4.2)}}& \textbf{46.0}& \textbf{30.2}& \textbf{6.7}& \textbf{29.8} \textcolor{red}{(+4.7)} \\ 
\hline
\end{tabular}





}
\label{baseline-on all}
\end{table*}

==> sec/table/inference_table.tex <==
\begin{table}[t]
\caption{Our framework outperforms existing methods in terms of both localization average mAP and inference speed.}
%with a 17.59\% increase in mAP, and inference speed, boasting a three-fold improvement.}
\renewcommand\arraystretch{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
  & \textbf{Label} & \textbf{mAP (0.3:0.7)}& \textbf{speed (img/s)} \\
  \hline
TriDet  & Action-Level& 69.3 & 6.67                  \\

Baseline& Video-Level & 35.8 & 1.64                  \\
\hline
\textbf{Baseline+NoCo} & Video-Level & 42.1 \textcolor{red}{(+6.3)} & 6.67 \textcolor{red}{(+5.03)}      \\
\hline
\end{tabular}
}
\label{inference-table}
\end{table}


==> sec/table/new-3.tex <==
%\input{sec/table/new-3}
\begin{table}[t]
\centering
\caption{Evaluation of each component of our method in IND dataset.}
\renewcommand\arraystretch{1.2}
\resizebox{230pt}{!}{

\begin{tabular}{c|cccc|ccc}

\hline
\multirow{2}{*}{} & \multirow{2}{*}{SAF} & \multirow{2}{*}{CPC} & \multirow{2}{*}{OPS} & \multirow{2}{*}{PMM} & \multicolumn{3}{c}{CASIA} \\ \cline{6-8} 
                  &                      &                      &                       &                      & I-F1   & P-F1   & Com-F1  \\ \hline
\Rmnum{1}               &                      &                      &                       &                      & 70.6   & 44.6   & 54.7    \\
\Rmnum{2}               & $\checkmark$                     &                      &                       &                      & 73.2   & 47.2   & 57.4    \\
\Rmnum{3}             &$\checkmark$                     & $\checkmark$                &                       &                      & 74.3   & 48.3   & 58.5    \\
\Rmnum{4}                & $\checkmark$            & $\checkmark$             & $\checkmark$                      &                      & 75.1   & 50.4   & 60.3    \\
\Rmnum{5}                 & $\checkmark$                     & $\checkmark$                   &$\checkmark$          & $\checkmark$                    & 77.3   & 50.6   & 61.2    \\ \hline
\end{tabular}



}
\label{AS1}
\end{table}



==> sec/table/new-4.tex <==
%\input{sec/table/new-4}
\begin{table}[t]
\centering
\caption{Evaluation of each component of our method in OOD dataset.}
\renewcommand\arraystretch{1.2}
\resizebox{190pt}{!}{


\begin{tabular}{c|cccc|ccc}

\hline
\multirow{2}{*}{} & \multirow{2}{*}{SAF} & \multirow{2}{*}{CPC} & \multirow{2}{*}{OPS} & \multirow{2}{*}{PMM} & \multicolumn{3}{c}{COVER} \\ \cline{6-8} 
                  &                      &                      &                       &                      & I-F1   & P-F1   & Com-F1  \\ \hline
\Rmnum{6}               &                      &                      &                       &                      & 20.4   & 23.1   & 21.7    \\
\Rmnum{7}              & $\checkmark$                     &                      &                       &                      & 49.6   & 37.6   & 42.8    \\
\Rmnum{8}            & $\checkmark$        & $\checkmark$          &                       &                      & 58.6   & 40.3   & 47.8    \\
\Rmnum{9}               & $\checkmark$     & $\checkmark$         & $\checkmark$     &                      & 65.2   & 44.7   & 53.0    \\
\Rmnum{10}             & $\checkmark$       & $\checkmark$      & $\checkmark$  & $\checkmark$      & 70.3   & 46.9   & 56.3    \\ \hline
\end{tabular}


}
\label{AS2}
\end{table}








==> sec/table/new-5.tex <==
%\input{sec/table/new-5}
\begin{table}[t]
\caption{Influence of Super-Resolution Method}
\renewcommand\arraystretch{1.2}
\resizebox{\linewidth}{!}{

\begin{tabular}{c|cccc|cc}
\hline
Methond & Param/M & FLOPs/G & PSNR  & SSIM & mAP-7 & mAP   \\ \hline
Bicubic & -       & -       & 31.16 & 0.79 & 68.89 & 56.21 \\
EDSR    & 43.09   & 823.34  & 33.64 & 0.86 & 70.51 & 57.69 \\
HSENet  & 21.70   & 306.31  & 33.85 & 0.87 & 70.61 & 57.77 \\
HAT-L   & 40.32   & 672.15  & 33.99 & 0.87 & 70.66 & 57.78 \\
TTST    & 18.94   & 317.68  & 34.31 & 0.87 & 70.70 & 57.81 \\ \hline
\end{tabular}



}
\label{Super_Resolution_compare}
\end{table}





